The partial vine copula: A dependence measure and approximation based on the simplifying assumption

Simplified vine copulas (SVCs), or pair-copula constructions, have become an important tool in high-dimensional dependence modeling. So far, specification and estimation of SVCs has been conducted under the simplifying assumption, i.e., all bivariate conditional copulas of the vine are assumed to be bivariate unconditional copulas. We introduce the partial vine copula (PVC) which provides a new multivariate dependence measure and which plays a major role in the approximation of multivariate distributions by SVCs. The PVC is a particular SVC where to any edge a j-th order partial copula is assigned and constitutes a multivariate analogue of the bivariate partial copula. We investigate to what extent the PVC describes the dependence structure of the underlying copula. We show that the PVC does not minimize the Kullback-Leibler divergence from the true copula and that the best approximation satisfying the simplifying assumption is given by a vine pseudo-copula. However, under regularity conditions, step-wise estimators of pair-copula constructions converge to the PVC irrespective of whether the simplifying assumption holds or not. Moreover, we elucidate why the PVC is the best feasible SVC approximation in practice.

==> preamble/Commands.tex <==
%%%%% COMMANDS %%%%
%--- general commands
\newcommand{\tc}{\textcolor}
\newcommand{\approxsign}[1]{\tilde{#1}}
\newcommand{\KL}[2]{D_{KL}(#1||#2)} % KL divergence
\newcommand{\parderiv}[2]{\partial_{#2}{#1}} % partial derivative
\newcommand{\as}{a.s.} 
\newcommand{\ivb}[1]{1\!\!1_{\{#1\}}} % iversion bracket
\renewcommand{\P}{\mathbb{P}}
\newcommand{\expec}{\mathbb{E}}
\newcommand{\var}{\mathbb{V}\text{ar}}
\newcommand{\cov}{\mathbb{C}\text{ov}}
\newcommand{\E}{{\cal E}}
\newcommand{\corr}{\mathbb{C}\text{orr}}
\newcommand{\indep}{\perp}
\newcommand{\R}{\mathbb{R}}
\newcommand{\eq}{\Leftrightarrow}
\newcommand{\imp}{\Rightarrow}
\newcommand{\std}[2]{\operatorname*{\!\!\!\!\!\!\!\!\phantom{_p}#1\phantom{_p}\!\!\!\!\!\!\!\!}_{#2}}

%--- vine copula related commands
\newcommand{\SPCC}{\mathfrak} % space of simplified pcc
\renewcommand{\SPCC}[1]{{\cal #1}^{\text{\tiny SVC}}} % space of simplified pcc
\newcommand{\idxset}{{\cal I}_\Mydim}
\newcommand{\parsign}[1]{#1^{\text{\tiny P}}} % partial copula
\newcommand{\pvc}[1]{#1^{\text{\tiny PVC}}} % j-th order partial copula
\newcommand{\condset}{S_{ij}} % conditioning variables
\newcommand{\sarg}[2]{S_{#1,#2}}
\newcommand{\cs}{|}
\newcommand{\ps}{;\,}
\renewcommand{\ps}{;\kern 0.08em}
%\renewcommand{\ps}{{\kern 0.06em} ;\kern 0.02em}
%\renewcommand{\ps}{;}

%--- specific commands for this paper
\newcommand{\idxz}{1}
\newcommand{\idxt}{3}
\newcommand{\idxlist}{1:3}
\newcommand{\idxo}{2}
\newcommand{\idxth}{4}
\newcommand{\idxf}{5}
\newcommand{\tmarg}{\theta_{12}}
\newcommand{\tpar}{\parsign{\theta}_{13\ps 2}}
\newcommand{\mdef}{m(u_\idxz,u_\idxt;\pvc{\theta}_{\idxz\idxt\ps \idxo})}
\newcommand{\hdef}[1]{h(#1;g)}
\newcommand{\fdef}[2]{f(#1,#2;\tpar)}
\newcommand{\Kdef}[1]{K(#1;\tpar)}
\newcommand{\Mydim}{K}
\newcommand{\Myx}{X}
\newcommand{\Gfun}[2]{\pvc{G}_{#1|\condset}(#2|u_{\condset})}
\newcommand{\Gfunt}[2]{\pvc{G}_{#1|\condset}(#2|t_{\condset})}


==> preamble/abbreviations.tex <==
\newcommand{\PVCA}{PVCA}
\newcommand{\pvca}{partial vine copula approximation}
\newcommand{\SVCA}{SVCA}
\newcommand{\svca}{simplified vine copula approximation}
\newcommand{\SVCM}{SVCM}
\newcommand{\svcm}{simplified vine copula model}
\newcommand{\SA}{simplifying assumption}
\newcommand{\dgp}{data generating process}
\renewcommand{\svcm}{simplified vine copula}
\renewcommand{\SVCM}{SVC}
\newcommand{\Svcm}{Simplified vine copula}
\renewcommand{\PVCA}{PVC}
\renewcommand{\pvca}{partial vine copula}


==> preamble/autoref_setup.tex <==
%%%%%%%%%% Define commands for automatic referencing
\let\orgautoref\autoref
\providecommand{\autorefs}
         {\def\sectionautorefname{Sections}%
         \def\subsectionautorefname{Sections}%
         \def\subfigureautorefname{Figures}%
         \def\mydefautorefname{Definitions}%
         \def\myexautorefname{Examples}%
         \def\mylemautorefname{Lemmas}%
         \def\myremautorefname{Remarks}%
         \def\mytheautorefname{Theorems}%
         \orgautoref}
         \providecommand{\appref}
{\def\subsectionautorefname{Appendix}%
         \orgautoref}
\renewcommand{\autoref}
        {\def\mydefautorefname{Definition}%
         \def\figureautorefname{Figure}%
         \def\subfigureautorefname{Figure}%
         \def\sectionautorefname{Section}%
         \def\subsectionautorefname{Section}%
         \def\mypropautorefname{Proposition}%
         \def\mycorautorefname{Corollary}%
         \def\subtableautorefname{Table}%
         \def\tableautorefname{Table}%
         \def\myexautorefname{Example}%
         \def\mylemautorefname{Lemma}%
         \def\myremautorefname{Remark}%
         \def\mytheautorefname{Theorem}%
         \orgautoref}
\makeatletter
\let\@autoref=\autoref
\renewcommand*{\autoref}[2][]{\ifthenelse{\equal{#1}{}}{\@autoref{#2}}{\hyperref[#1]{\begin{NoHyper}\@autoref{#2}~\subref{#1}\end{NoHyper}}}\xspace}
\makeatother


==> preamble/options.tex <==

\excludeversion{note}
\setlength{\emergencystretch}{1em}

%%%%%%%%%% COUNTERS ETC
%\iffalse
\numberwithin{myprop}{section}
\numberwithin{mycor}{section}
\numberwithin{myex}{section}
\numberwithin{mydef}{section}
\numberwithin{mylem}{section}
\numberwithin{myrem}{section}
\numberwithin{mythe}{section}
%\fi
\numberwithin{equation}{section}


==> preamble/preamble.tex <==
%%%% PACKAGES %%%%
\RequirePackage[numbers]{natbib}
\usepackage{amssymb}
\usepackage[bookmarksdepth,colorlinks=true]{hyperref}
\usepackage{bookmark}
\usepackage[hyperref,thmmarks]{ntheorem} % should be loaded after hyperref, there are also compatibility issues with maththools
\usepackage{graphicx}
\usepackage[labelsep=newline,font=small,labelfont=bf,singlelinecheck=false]{caption}
\usepackage{xspace}
\usepackage{ifthen}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{enumerate}
\usepackage{versions}

%%%%%%%%%% COMMANDS
\input{preamble/Commands}

%%%% OPTIONS %%%%
\input{preamble/theorem_setup}
\input{preamble/autoref_setup}
\input{preamble/options}
\captionsetup[figure]{singlelinecheck=on, labelsep=colon}

%%%% MISC %%%%
\input{preamble/abbreviations}
\hyphenation{Ar-chi-me-dean}
\newcommand\tagging{\addtocounter{equation}{1}\tag{\theequation}}
\def\RefEqual#1{\stackrel{\text{\tiny\makebox[0pt]{#1}}}{=}}




==> preamble/theorem_setup.tex <==


\theoremstyle{break} % defines the style, 'break' inserts a line break before the %text begins
%\theorembodyfont{\slshape} % can be \rmfamily (default), \upshape, 
\theoremseparator{} % specifies the separator after the name of the theorem
\newtheorem{myprop}{Proposition}
\newtheorem{mycor}{Corollary}
\newtheorem{mydef}{Definition}
\newtheorem{mylem}{Lemma}
\newtheorem{myrem}{Remark}
\newtheorem{mythe}{Theorem}
%\theorembodyfont{\rmfamily}
\newtheorem{myex}{Example}

\theorembodyfont{\rmfamily}
\theoremstyle{nonumberplain}
\theoremseparator{.}
\theoremsymbol{\ensuremath{\blacksquare}}
\newtheorem{myproof}{Proof}

